Federated Prompting and Chain-of-Thought Reasoning for Improving LLMs Answering

We investigate how to enhance answer precision in frequently asked questions posed by distributed users using cloud-based Large Language Models (LLMs). Our study focuses on a typical situations where users ask similar queries that involve identical mathematical reasoning steps and problem-solving procedures. Due to the unsatisfactory accuracy of LLMs' zero-shot prompting with standalone questions, we propose to improve the distributed synonymous questions using Self-Consistency (SC) and Chain-of-Thought (CoT) techniques. Specifically, we first retrieve synonymous questions from a crowd-sourced database and create a federated question pool. We call these federated synonymous questions with the same or different parameters SP-questions or DP-questions, respectively. We refer to our methods as Fed-SP-SC and Fed-DP-CoT, which can generate significantly more accurate answers for all user queries without requiring sophisticated model-tuning. Through extensive experiments, we demonstrate that our proposed methods can significantly enhance question accuracy by fully exploring the synonymous nature of the questions and the consistency of the answers.

==> OK/federated_learning.tex <==
\textbf{Federated learning}


The first equation is known as the client-level objective, and it aims to minimize the average loss over all of the clients in a distributed system. In this equation, $w$ is the model parameter that we want to learn, and $f(w)$ is the average loss across all clients. The function $f_i(w)$ is the loss function for client $i$, and $n$ is the total number of clients in the system. The goal of this equation is to find the optimal $w$ that minimizes the overall loss across all clients.

\begin{equation}
\min_{w\in \mathbb{R}^d} \sum_{k=1}^{K}\frac{n_k}{n}F_k(w), \quad \text{where} \quad F_k(w)=\frac{1}{n_k}\sum_{i\in P_k}f_i(w) \tag{2}
\end{equation}

The second equation is known as the server-level objective. It is a equation of the federated learning optimization problem, where the goal is to learn a global model parameter vector, denoted by $w$, by minimizing the average loss across all participating clients. The clients are divided into $K$ non-overlapping groups, denoted by $P_k$, and each client $i$ within a group $k$ has a local dataset of size $n_k$. The loss function $f_i(w)$ measures the discrepancy between the predictions of the model and the ground truth labels on the local dataset of client $i$. The function $F_k(w)$ computes the average loss of the clients in group $k$, which is a weighted average of the local losses, where the weight is proportional to the number of samples each client contributes. The objective is to find the global model parameter $w$ that minimizes the average of the group-wise losses.
